Becoming the Super Turker: Increasing Wages via a Strategy from High Earning Workers

Crowd markets have traditionally limited workers by not providing transparency information concerning which tasks pay fairly or which requesters are unreliable. Researchers believe that a key reason why crowd workers earn low wages is due to this lack of transparency. As a result, tools have been developed to provide more transparency within crowd markets to help workers. However, while most workers use these tools, they still earn less than minimum wage. We argue that the missing element is guidance on how to use transparency information. In this paper, we explore how novice workers can improve their earnings by following the transparency criteria of Super Turkers, i.e., crowd workers who earn higher salaries on Amazon Mechanical Turk (MTurk). We believe that Super Turkers have developed effective processes for using transparency information. Therefore, by having novices follow a Super Turker criteria (one that is simple and popular among Super Turkers), we can help novices increase their wages. For this purpose, we: (i) conducted a survey and data analysis to computationally identify a simple yet common criteria that Super Turkers use for handling transparency tools; (ii) deployed a two-week field experiment with novices who followed this Super Turker criteria to find better work on MTurk. Novices in our study viewed over 25,000 tasks by 1,394 requesters. We found that novices who utilized this Super Turkers' criteria earned better wages than other novices. Our results highlight that tool development to support crowd workers should be paired with educational opportunities that teach workers how to effectively use the tools and their related metrics (e.g., transparency values). We finish with design recommendations for empowering crowd workers to earn higher salaries.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> trash.tex <==
Requesters with no transparency ratings are likely to be newcomers on MTurk, as professional requesters, generally, have longer histories concerning posted HITs; and hence a higher likelihood to have been previously evaluated on transparency tools. 


the effect of having novices adopt different criteria, as well as engage in in-depth interviews with novices and Super Turkers to further understand transparency in crowd markets. Related it might also be interesting to study the amount of time it takes novices to adopt on their own some of the Super Turker strategies.
% \subsection{Design Implications.} 


%We found that novice workers who followed the strategy of Super Turkers earned a better hourly wage than novices working independently. Nonetheless, the hourly wage of novices still remained too low. One potential reason might be that novices need to develop certain digital skills to adequately execute the strategy.  Although the strategy was relatively simple, learning how to follow the strategy might be something that  cannot be reached in one step. Future work could study the long term impact of having novices follow strategies from Super Turkers. Novice workers might need a longer time period to learn how to appropriate and integrate the instructions from Super Turkers into their work. We plan to create tools that guide novices on how to follow Super Turker strategies and we will study novices' working patterns long term. Another of the reasons why novices might have had low wages is that there are likely other hidden variables involved (variables that do not necessarily involve adequately using transparent information.)  A person's working time on MTurk can in general be separated into: a) time spent searching for tasks to do; and b) time spent completing a task. Reducing the working time represents increasing the hourly wages because crowd workers can do more tasks under a specific time frame. Strategies for using transparency might help reduce the time workers spend searching for tasks, but they might not reduce the time workers spend completing a task. Researchers have been exploring tools that help workers complete tasks faster by helping workers to develop their skills \cite{chiang2018crowd,lundgard2018bolt}. Future work could explore tools that help workers to  reduce both the time they spend searching for work and the time they spend completing tasks to foster better wages and professional growth on MTurk.



%Notice that it was possible that following the strategy could have lead novices to potentially reduce their wages. In our instructions, we advised novices to use their common sense and if they felt that doing the strategy would hurt them in any way to not follow it. We also told novices that if they experienced any problems when following the strategy to please contact us. We were willing to compensate workers who might have experienced any losses. Future work could study why certain novices decide to not follow a strategy from Super Turkers. What barriers or problems do they encounter?  

%Our investigation also focused on understanding how a strategy from Super Turkers played out in the wild when adopted by novices. Future work could conduct longitudinal studies and engage in in-depth interviews with Super Turkers to understand the different types of strategies that they have and also conduct analysis of how such strategies are adopted by novices long term. 

% novice workers try to build a different strategy to select fair payment tasks on their own, but the process of trial and error would reduce their income.
% Therefore, it is particularly important to guide novice workers on how to overcome the obstacles of low-income.

%\section{Conclusion}


%We examined how Super Turkers use transparent information to select lucrative tasks and earn high hourly wages. Our study reveals that Super Turkers to avoid underpaid crowd tasks and reduce their unpaid working time use transparency to identify a task's expected hourly payment and have an overview of a requesters reputation, especially how fair they are. Armed with this knowledge,  we conducted a two-week experiment in the real world to understand the impact of having novices follow these strategies. We traced the working history of 99 novice workers on Amazon Mechanical Turk who were placed into two conditions: an experimental condition where they were instructed to follow the strategies and a control condition where workers worked independently. We identified that novice workers did not discover or generally use the Super Turker strategies on their own and novice workers can increase their hourly wage if they follow how Super Turkers use transparency tools. Our results demonstrate that providing transparent data is not enough for helping novice workers to increase their salary. Novices also need some background on how to effectively use transparency.











%This showcases that following the decision-making criteria from Super Turkers' can improve the salaries of novices (even in potentially bad market conditions). By having novices only look at three transparency variables and use that to make rapid decisions of what work to perform, we were able to reduce the search times of novices and increase their wages (as they spent less time over analyzing the different transparency data available.)
%and focused more on paid labor.) 
 
 
 The tutorials could also be data driven based on the behavior of Super Turkers to facilitate their creation.


Through data analysis of Super Turkers' process for using transparency information, we computationally developed a set of criteria for novices to follow. We then investigate what happens when novices in the wild follow the criteria to find work on MTurk. 


, i.e., crowd workers with less than 500 completed HITs (human-intelligence-tasks)

arising from gaps in regulatory models governing patient safety
%First, we began this research by studying and familiarizing ourselves with Super Turkers. For almost a year we watched live streams on YouTube and Twitch of Super Turkers in action \cite{rodney_2017}. We also paid Super Turkers to make instructional videos where they performed HITs on camera and described their best practices for using transparency tools.
%We realized that Super Turkers had a variety of criteria that they valued and utilized when deciding which tasks to perform. It was a difficult undertaking for us to quantify the most popular ones. However, by conducting surveys of Super Turkers to obtain exactly how they utilized transparency tools, we achieved a set of criteria that was based on the majority of Super Turker behavior which has been demonstrated to be an appropriate and valid method.


The values of the transparency metrics in the criteria that we developed (e.g., \$8.29 USD/h or 3.69) came from the averaged values of what Super Turkers inputted for those metrics when creating their criteria flowcharts. 

condenses the recent and most relevant research done in the 3D printing assitive technology space, and helps to start visualizing where current knowledge gaps exist



(``always'' and ``most of the time'')


Note that we did not provide open-ended questions because our goal is to find the common use strategy about how to use the public information. 
%a market is transparent if much is known by many about: What products and services or capital assets are available, market depth (quantity available), what price, and where. Transparency is important since it is one of the theoretical conditions required for a free market to be efficient. Price transparency can, however, lead to higher prices. For example, if it makes sellers reluctant to give steep discounts to certain buyers (e.g. disrupting price dispersion among buyers), or if it facilitates collusion, and price volatility is another concern.[1] A high degree of market transparency can result in disintermediation due to the buyer's increased knowledge of supply pricing.


